Machine Unlearning of Federated Clusters

Federated clustering (FC) is an unsupervised learning problem that arises in a number of practical applications, including personalized recommender and healthcare systems. With the adoption of recent laws ensuring the "right to be forgotten", the problem of machine unlearning for FC methods has become of significant importance. We introduce, for the first time, the problem of machine unlearning for FC, and propose an efficient unlearning mechanism for a customized secure FC framework. Our FC framework utilizes special initialization procedures that we show are well-suited for unlearning. To protect client data privacy, we develop the secure compressed multiset aggregation (SCMA) framework that addresses sparse secure federated learning (FL) problems encountered during clustering as well as more general problems. To simultaneously facilitate low communication complexity and secret sharing protocols, we integrate Reed-Solomon encoding with special evaluation points into our SCMA pipeline, and prove that the client communication cost is logarithmic in the vector dimension. Additionally, to demonstrate the benefits of our unlearning mechanism over complete retraining, we provide a theoretical analysis for the unlearning performance of our approach. Simulation results show that the new FC framework exhibits superior clustering performance compared to previously reported FC baselines when the cluster sizes are highly imbalanced. Compared to completely retraining K-means++ locally and globally for each removal request, our unlearning procedure offers an average speed-up of roughly 84x across seven datasets. Our implementation for the proposed method is available at https://github.com/thupchnsky/mufc.

==> sec_machine_unlearning.tex <==
\vspace{-3pt}
\section{Machine Unlearning via Specialized Seeding}\label{sec:mu}
\vspace{-3pt}
%Before the introduction of the complete procedure of our unlearning algorithm for federated clusters, 
We first exhibit an intuitive exact unlearning mechanism (Alg.~\ref{alg:mu_kpp}) for $K$-means clustering in the centralized setting, which will be later on used for the unlearning procedure of client-side clustering in the FC framework described in Section~\ref{sec:ufc}. The idea of Alg.~\ref{alg:mu_kpp} is straightforward: one needs to rerun the $K$-means++ initialization, corresponding to retraining, only when the current centroid set $\mathbf{C}$ contains one or more of the points that are requested to be removed. This results from two observations. First, since the centroids chosen through $K$-means++ initialization are true data points, the updated centroid set $\mathbf{C}^\prime$ returned by Alg.~\ref{alg:mu_kpp} are guaranteed to contain no information about the data points that have been removed. Furthermore, as we will explain in the next section, Alg.~\ref{alg:mu_kpp} also satisfies the exact unlearning criterion (defined in Section \ref{sec:prelim}).

\begin{wrapfigure}[22]{L}{0.47\textwidth}
\begin{minipage}{0.47\textwidth}
\vspace{-13pt}
\begin{algorithm}[H]
   \caption{Unlearning via $K$-means++ Init.}
   \label{alg:mu_kpp}
   \begin{algorithmic}[1]
    \STATE \textbf{input:} Dataset $\mathcal{X}$, centroid set $\mathbf{C}$ obtained by $K$-means++ initialization on $\mathcal{X}$, removal request set $\mathcal{X}_R=\{x_{r_1},\ldots,x_{r_R}\}$.
    \IF{$c_j\notin \mathcal{X}_R\;\forall c_j\in\mathbf{C}$}
    \STATE $\mathbf{C}^\prime \leftarrow \mathbf{C}$
    \ELSE
    \STATE $i\leftarrow (\argmin_j c_j\in \mathcal{X}_R) - 1$
    \IF{$i=0$}
    \STATE $\mathbf{C}^\prime \leftarrow \varnothing$, $\mathcal{X}^\prime\leftarrow \mathcal{X}\backslash\mathcal{X}_R$.
    \ELSE
    \STATE $\mathbf{C}^\prime \leftarrow \{c_1,\ldots,c_i\}$, $\mathcal{X}^\prime\leftarrow \mathcal{X}\backslash\mathcal{X}_R$.
    \ENDIF
    \FOR{$j = i+1,\ldots,K$}
      \STATE Sample $x$ from $\mathcal{X}^\prime$ with prob
        $\frac{d^2(x,\mathbf{C}^\prime)}{\phi_c(\mathcal{X}^\prime;\mathbf{C}^\prime)}$.
      \STATE $\mathbf{C}^\prime \leftarrow\mathbf{C}^\prime\cup \{x\}$.
    \ENDFOR
    \ENDIF
    \RETURN $\mathbf{C}^\prime$
  \end{algorithmic}
\end{algorithm}
\end{minipage}
\vspace{0.1in}
\end{wrapfigure}

\subsection{Performance Analysis}
To verify that Alg.~\ref{alg:mu_kpp} is an exact unlearning method, we need to check that $\mathbf{C}^\prime$ is probabilistically equivalent to the models generated by rerunning the $K$-means++ initialization process on $\mathcal{X}^\prime$, the set of point remaining after removal. This is guaranteed by Lemma~\ref{lma:mu_kpp}, and a formal proof is provided in Appendix~\ref{app:mu_kpp}.

% Suppose that one would like to unlearn the data point $x_i$ from the clustering model represented by an initial centroid set $\mathbf{C}$. For the first  chosen centroid $c_1$ in $\mathbf{C}$, there are only two possibilities: $c_1=x_i$ and $c_1\neq x_i$. In the first case, we will have to re-run the initialization over $\mathcal{X}^\prime$, which is retraining the model. In the second case, since we know $c_1\neq x_i$, the probability of choosing $c_1$ from $\mathcal{X}$ as the first centroid becomes the conditional probability $\mathbb{P}($choose $c_1$ from $\mathcal{X}$ as the first centroid$|c_1\neq x_i)=\frac{1}{n-1}=\mathbb{P}($choose $c_1$ from $\mathcal{X}^\prime$ as the first centroid$)$, where $n$ is the number of data points in $\mathcal{X}$. Therefore, the first centroid $c_1^\prime$ returned by Alg.~\ref{alg:mu_kpp} can always be viewed as the first centroid obtained by re-running the initialization over $\mathcal{X}^\prime$. This can be generalized for $c_j\;\forall j\in[K]$ and $\mathcal{X}_R$ of arbitrary sizes. Since Alg.~\ref{alg:mu_kpp} is an exact unlearning method, we can have the performance guarantees in Lemma~\ref{lma:mu_kpp} based on Theorem 1.1 of~\citet{vassilvitskii2006k}.%, which shows that our unlearning mechanism can achieve the same performance as re-running the initialization over $X^\prime$.
\begin{lemma}\label{lma:mu_kpp}
For any set of data points $\mathcal{X}$ and removal set $\mathcal{X}_R$, assuming that the remaining dataset is $\mathcal{X}^\prime=\mathcal{X}\backslash\mathcal{X}_R$ and the centroid set returned by Alg.~\ref{alg:mu_kpp} is $\mathbf{C}^\prime$, we have 
$$
\mathbb{P}(\mathcal{U}(\mathcal{A}(\mathcal{X}), \mathcal{X}, \mathcal{X}_R)=\mathbf{C}) = \mathbb{P}(\mathcal{A}(\mathcal{X}^\prime)=\mathbf{C});\; \mathbb{E}(\phi_c(\mathcal{X}^\prime;\mathbf{C}^\prime))\leq 8(\ln K+2)\phi^*_c(\mathcal{X}^\prime),
$$
where $\mathcal{A}$ represents Algorithm~\ref{alg:fl_clustering} and $\mathcal{U}$ represents the unlearning mechanism in Algorithm~\ref{alg:mu_kpp}.
\end{lemma}
% Proof of Lemma \ref{lma:mu_kpp} is in Appendix \ref{app:mu_kpp}.
\subsection{Complexity Analysis}
%The goal of machine unlearning is to reduce the removal time complexity while keeping performance competitive with retraining. 
We next present our analytical results for the expected time complexity for removing a batch of $R$ data points by our Alg.~\ref{alg:mu_kpp}. For this, we consider both scenarios of random removal and adversarial removal.  While the analysis for random removal is relatively easier, we note that the analysis for adversarial removal essentially requires us to address the issue of removal requests that would force frequent retraining from scratch. In this regard, we state two assumptions concerning optimal cluster sizes and outliers, to characterize the worst-case scenario in adversarial removal setting. 
\begin{assumption}\label{def:imbalance}
Let $\epsilon_1=\frac{n}{K s_{\min}}$ be a constant denoting \emph{cluster size imbalance,} where $s_{\min}$ equals the size of the smallest cluster in the optimal clustering; when $\epsilon_1=1$, all clusters are of size $\frac{n}{K}$.
\end{assumption}
\begin{assumption}\label{def:outlier}
% Assume that the whole dataset $X$ consists of two disjoint part: true cluster points $X_t$ and outliers $X_o$ \textcolor{red}{not sure what you call outlier here - is below the definition? if yes, this should be made more clear...}. For each point $x_i \in X_o$ and a constant $\epsilon_2\geq 1$, \textcolor{red}{it satisfies that??}
Assume that $\epsilon_2\geq 1$ is a fixed constant. An outlier $x_i$ in $\mathcal{X}$ satisfies $\|x_i-c_j^*\|\leq \|x_i-c_k^*\|, \forall k\in[K]$ and  $\|x_i-c_j^*\| > \sqrt{{\epsilon_2\phi_c^*(\mathcal{C}_j^*)}/{|\mathcal{C}_j^*|}}$.
\end{assumption}

% \begin{remark*}
% The requirement on the minimum cluster size in Assumption \ref{def:imbalance} is pretty common in theoretical analysis for clustering problems \cite{chien2018query,ginart2019making,dennis2021heterogeneity} to exclude the worst case happening on tiny clusters which may otherwise lead to significant changes. The notion of outliers used in Assumption \ref{eq:outlier} is considered to capture the data points that are well-separated
% from all “regular” clusters: the distance between an outlier and its closest centroid is larger than a scaled proxy for the empirical standard deviation of the average distance between the cluster points and that centroid \cite{dennis2021heterogeneity,chien2018query}.     
% \end{remark*}

\begin{comment}
Assumptions~\ref{def:imbalance} and~\ref{def:outlier} can be used to derive an expression for the probability of $x_i\in\mathbf{C}$ when $x_i$ needs to be unlearned, which equals the probability of retraining with $\mathcal{X}^\prime$.
\begin{lemma}\label{lma:retrain_prob}
Assume that the number of data points in $\mathcal{X}$ is $n$ and the probability of the dataset containing at least one outlier is upper bounded by $O\left({1}/{n}\right)$. Let $\mathbf{C}$ be the centroid set obtained by running $K$-means++ on $\mathcal{X}$. For unlearning a data point $x_i \in \mathcal{X}$ we have that for random removal: $\mathbb{P}(x_i\in\mathbf{C})<O\left({K}/{n}\right)$; for adversarial removal: $\mathbb{P}(x_i\in\mathbf{C})<O\left({K^2\epsilon_1\epsilon_2}/{n}\right)$.
\end{lemma}
\end{comment}

Under Assumptions \ref{def:imbalance} and \ref{def:outlier}, we arrive at an estimate of the expected removal time as shown in Theorem~\ref{thm:expected_removal_time} below. Quite notably, the results are independent of the problem size $n$. %This makes the approach especially suitable for large-scale datasets.

\begin{theorem}\label{thm:expected_removal_time}
% Assume that the number of data points in $\mathcal{X}$ is $n$ and the probability of the dataset containing at least one outlier is upper bounded by $O\left({1}/{n}\right)$. Algorithm~\ref{alg:mu_kpp} supports removing $R$ points with time $O(RK^2d)$ in expectation for random removals, and with time $O(RK^3\epsilon_1\epsilon_2d)$ in expectation for adversarial removals. The time complexity of complete retraining equals $O(nKRd)$.
Assume that the number of data points in $\mathcal{X}$ is $n$ and the probability of the data set containing at least one outlier is upper bounded by $O\left({1}/{n}\right)$. Algorithm~\ref{alg:mu_kpp} supports removing $R$ points within single request with time $\min\{O(RK^2d), O(nKd)\}$ in expectation for random removals, and with time $\min\{O(RK^3\epsilon_1\epsilon_2d), O(nKd)\}$ in expectation for adversarial removals. The time complexity of complete retraining equals $O(nKd)$.
\end{theorem}

\begin{remark*}
Due to the distance-based $K$-means++ initialization procedure used for local clustering, the existence of outliers in the data set would inevitably lead to higher retraining probability. This is because outliers are more likely to lie in the initial set of centroids. Hence, for analytical purposes, we assume in Theorem \ref{thm:expected_removal_time} that the probability of the data set containing at least one outlier is upper bounded by $O\left({1}/{n}\right)$. This is not overly restrictive as there exist many different approaches for
removing outliers for clustering problems \cite{chawla2013k,gan2017k,hautamaki2005improving}, which effectively reduce the probability of outliers to negligible values and can be used as data preprocessing procedure within our framework.
\end{remark*}


\subsection{Unlearning Federated Clusters}\label{sec:ufc}
We next describe the complete unlearning algorithm for our FC framework, which uses Algorithm~\ref{alg:mu_kpp} as one component for client-side clustering. In FL setting, data only resides on clients, and thus the basic assumption of federated unlearning is that the removal requests will only appear at client side, and the removal set will not be known to other unaffected clients and the server. Here we consider two types of removal requests in FC setting: removing $R$ points from one client $l$ (cross-silo, single-client removal), and removing all data points from $R$ clients $l_1,\ldots,l_R$ (cross-device, multi-client removal). For the case where multiple clients want to unlearn only a part of their data, the approach is similar to that of single-client removal and can be estimated by simple union bounds.

The unlearning procedure is depicted in Algorithm~\ref{alg:mu_fl}. For single-client removal, the algorithm will first perform unlearning on client $l$ following Algorithm~\ref{alg:mu_kpp}. If the client's local clustering changes (i.e., client $l$ reruns the initialization), it will generate a new $q^{(l)}$ and send it to the server through the SCMA scheme. Then the server will rerun the clustering procedure with the new aggregated vector $q^\prime$ and generate a new set of global centroids $\mathbf{C}_s^\prime$. Note that other clients do not need extra computation during this process. For multi-client removal, affected clients will send $q^{(l)}=\mathbf{0}$ and send them to the server through the SCMA scheme. Again, the server will rerun the clustering procedure and generate a new set of global centroids. In this case, no clients need extra computation during this process.


Following the same reasoning as the case of centralized unlearning in Lemma~\ref{lma:mu_kpp}, we can show that Algorithm~\ref{alg:mu_fl} is also an exact unlearning method.
% in Lemma~\ref{lma:mu_kpp}, one can show that the result of Theorem~\ref{thm:fl_performance_quantize} also holds for the remaining data set $\mathcal{X}^\prime$ after running the unlearning procedure in Algorithm~\ref{alg:mu_fl}.

\textbf{Removal time complexity.} For single-client removal, we know from Theorem~\ref{thm:expected_removal_time} that the expected removal time complexity of client $l$ is $\min\{O(RK^2d), O(n^{(l)}Kd)\}$ and $\min\{O(RK^3\epsilon_1\epsilon_2d), O(n^{(l)}Kd)\}$ for random and adversarial removals, respectively. $n^{(l)}$ denotes the number of data points on client $l$. Other clients do not require additional computations, since their centroids will not be affected by the removal requests. Meanwhile, the removal time complexity for the server is upper bounded by $O(K^2LTd)$, where $T$ is the maximum number of iterations of Lloyd's algorithm at the server before convergence.

For multi-client removal, no client needs to perform additional computations, and the removal time complexity for the server equals $O((L-R)K^2Td)$.

\begin{wrapfigure}[24]{L}{0.5\textwidth}%{0.5\textheight}
\begin{minipage}{0.5\textwidth}
\vspace{-23pt}
\begin{algorithm}[H]
   \caption{Unlearning of Federated Clusters}
   \label{alg:mu_fl}
   \begin{algorithmic}[1]
    \STATE \textbf{input:} Dataset $\mathcal{X}$ distributed on $L$ clients ($\mathcal{X}^{(1)},\ldots,\mathcal{X}^{(L)}$), ($\mathbf{C}^{(l)}, \mathcal{X}_s, q, \mathbf{C}_s$) obtained by Algorithm~\ref{alg:fl_clustering} on $\mathcal{X}$, removal request set $\mathcal{X}_R^{(l)}$ for single-client removal or $\mathcal{L}_R$ for multi-client removal.
    \IF{single-client removal}
    \STATE Run Algorithm~\ref{alg:mu_kpp} on client $l$ and update $q^{(l)}$ if client $l$ has to perform retraining.
    \ELSE
    \STATE $q^{(l)}\leftarrow\mathbf{0}$ on client $l$, $\forall l\in\mathcal{L}_R$.
    \ENDIF
    \STATE Securely sum up $q^{(l)}$ at server by Algorithm~\ref{alg:fl_secure}, with the aggregated vector denoted as $q^\prime$.
    \IF{$q^\prime=q$}
    \STATE $\mathbf{C}_s^\prime\leftarrow \mathbf{C}_s$.
    \ELSE
    \STATE Generate $\mathcal{X}_s^\prime$ with $q^\prime$.
    \STATE Run full $K$-means++ at the server with $\mathcal{X}_s^\prime$ to obtain $\mathbf{C}_s^\prime$.
    \ENDIF
    \RETURN Client centroid sets $\mathbf{C}^{(l)\prime}$, server data $\mathcal{X}_s^\prime, q^\prime$ and centroids $\mathbf{C}_s^\prime$.
  \end{algorithmic}
\end{algorithm}
\end{minipage}
\end{wrapfigure}
